Single-cell Subcellular Protein Localisation Using Novel Ensembles of Diverse Deep Architectures

Unravelling protein distributions within individual cells is key to understanding their function and state and indispensable to developing new treatments. Here we present the Hybrid subCellular Protein Localiser (HCPL), which learns from weakly labelled data to robustly localise single-cell subcellular protein patterns. It comprises innovative DNN architectures exploiting wavelet filters and learnt parametric activations that successfully tackle drastic cell variability. HCPL features correlation-based ensembling of novel architectures that boosts performance and aids generalisation. Large-scale data annotation is made feasible by our "AI-trains-AI" approach, which determines the visual integrity of cells and emphasises reliable labels for efficient training. In the Human Protein Atlas context, we demonstrate that HCPL defines state-of-the-art in the single-cell classification of protein localisation patterns. To better understand the inner workings of HCPL and assess its biological relevance, we analyse the contributions of each system component and dissect the emergent features from which the localisation predictions are derived.

==> email.tex <==
Dear Dr Doerr

I am writing to briefly introduce my team and our recent work on a method for subcellular protein localisation within individual cells, which we intend to submit to Nature Methods. 

There is much interest in unravelling protein distributions within individual cells, as it helps to understand cell function and state and is indispensable to developing new treatments. This, and a lack of published solutions, motivated us to develop HCPL - a novel system to localise proteins at a subcellular level. It processes high-resolution confocal microscopy images to segment individual cells, assesses their visual integrity, and predicts protein localisation patterns. Importantly, HCPL makes large-scale single-cell data annotation feasible by helping to avoid the need to hand-label individual cells. HCPL currently defines state-of-the-art in the single-cell classification of protein localisation patterns.

Despite recent advances in automated cell image analysis and increasing demand for efficient methods, the development in the area of automated subcellular protein localisation for individual cells has been lacking with no published methods available.  The image-level methods (such as “Analysis of the Human Protein Atlas Image Classification competition”, published in your journal) are not applicable to individual cell analysis because of their unacceptably poor performance. 

In the manuscript, we aim to bridge this knowledge gap and present a novel approach that overcomes the major bottlenecks of the subcellular analysis, such as the lack of accurate annotations, substantial variability in the appearance of cells and challenging imaging conditions. 

My team has been working on core methods in ML for image analysis for the past 25 years, and we proposed the core algorithms adapted for this work, such as Hybrid Deep Neural Networks, a learnable activation layer, and multi-stream architectures.

Given the profile of your journal, its scope covering single-cell analysis and imaging methodologies, and the importance of the problem we address, we believe our manuscript will be of interest to Nature Methods readers and valuable addition to the journal. 

Please note that this manuscript was published as a preprint on 19 May 2022 (https://arxiv.org/abs/2205.09841) 

Aiming to publish in Nature Methods, we would appreciate any comments or questions that you may have on our manuscript. We will address your suggestions before submission.  

% Ask which paper format is most suitable

With regards,
Prof...
